SCALE-UP: An Efficient Black-box Input-level Backdoor Detection via Analyzing Scaled Prediction Consistency

Deep neural networks (DNNs) are vulnerable to backdoor attacks, where adversaries embed a hidden backdoor trigger during the training process for malicious prediction manipulation. These attacks pose great threats to the applications of DNNs under the real-world machine learning as a service (MLaaS) setting, where the deployed model is fully black-box while the users can only query and obtain its predictions. Currently, there are many existing defenses to reduce backdoor threats. However, almost all of them cannot be adopted in MLaaS scenarios since they require getting access to or even modifying the suspicious models. In this paper, we propose a simple yet effective black-box input-level backdoor detection, called SCALE-UP, which requires only the predicted labels to alleviate this problem. Specifically, we identify and filter malicious testing samples by analyzing their prediction consistency during the pixel-wise amplification process. Our defense is motivated by an intriguing observation (dubbed scaled prediction consistency) that the predictions of poisoned samples are significantly more consistent compared to those of benign ones when amplifying all pixel values. Besides, we also provide theoretical foundations to explain this phenomenon. Extensive experiments are conducted on benchmark datasets, verifying the effectiveness and efficiency of our defense and its resistance to potential adaptive attacks. Our codes are available at https://github.com/JunfengGo/SCALE-UP.

==> preliminary.tex <==
\section{Preliminaries}
\label{sec:preliminaries}



\subsection{Threat Model}
\label{sec:threat_model}
Our considered threat model contains two parts: the \textit{adversary} and the \textit{defender}. Consistent with previous work~\citep{DBLP:journals/corr/abs-1708-06733,Trojannn,chen,ISSBA}, the attacker can inject arbitrary amounts of poisoned samples in the training phase to ensure the attack efficacy. As for the defender, we consider a threat model with the weakest assumption, where both the poisoned training samples and target DNN's parameters are inaccessible. The defender can only obtain the final predictive label for each input. The defender treats the target black-box model as infected and aims to identify the backdoored sample at its inference phase. 

\subsection{Problem Formulation}
Consistent with previous work~\citep{nc,guo2019tabor,dong2021black,wang2020practical,karm}, we deem a DNN is infected with backdoor if one can cause the DNN misclassify any benign input into a target label when adding a specific modification(trigger). Such a specific triggeer is pre-defined by the attacker. Without loss of generality, for each benign sample $x\in\mathbb{R}^{n}$, the corresponding backdoored sample can be formulated as:

\begin{equation}
    \label{eq:backdoor_sample}
    \hat{x} = x+g(x), \quad ||g(x)||_{\infty} \leq \epsilon ~~ \forall x
\end{equation}

where, the generator function $g$ takes each input $x$ and generates an imperceptible trigger. The static trigger scenario widely considered by ~\citep{nc,karm,wang2020practical,DBLP:journals/corr/abs-1708-06733,guo2019tabor} can be treated as a special case for \cref{eq:backdoor_sample}, where $g(x) = m\odot(\bigtriangleup-x)$, thus $\hat{x} = (1-m)\odot x+m\odot\bigtriangleup$, where $x \in \mathbb{R}^{n}$ represents the static backdoor trigger and $\odot$ represents the element-wise product. $m \in \{0,1\}^{n}$ is a binary mask that ensures the trigger's position and is applied consistently across any sample.

We define $f(\cdot,;\theta)$ as the target DNN with parameters $\theta$, which takes $x$ as input and gives the corresponding predictive label $y$. We uses $\phi(x,y;\theta)$ as the softmax probability for $x$ predicted as $y$ by $f(\cdot;\theta)$. The attacker make $f$ to misclassify each $\hat{x_{i}}$ as target label $y_{t}$ through optimizing:
\begin{equation}
    \label{eq:training}
    \hat{\theta} = \argmin_{\theta} \sum_{i=1}^{N_{o}} \ell(\phi(x_{i},y_{i};\theta),y_{i}) + \sum_{j=1}^{N_b}\ell(\phi(\hat{x_{j}},y_t;\theta),y_t),
\end{equation}
where the attacker uses $N_{o}$ benign samples and $N_{b}$ poisoned samples. $\ell(\cdot)$ represents the cross-entropy loss and $\{x_{i},y_{i}\}_{i=1}^{N_{o}}$ are pairs of benign samples and ground truth labels. As for the inference phase, $f(\hat{x}) = y_{t}$.

\subsection{Black-box Sample-Level backdoor Detection and Its challenges}
Following previous work~\citep{strip,rethinking,frequency,deepweep}, we study the problem that how to identify the backdoored and benign samples at the inference time for $f(\cdot;\theta)$(if infected), we formulate such problem as `training' a binary classifiers $\mathcal{D}$:
\begin{equation}
    \label{eq:sample_wise}
    \mathcal{D}_{f(\cdot;\theta)}(x) =  \begin{cases}
    1, \text{backdoored}\\
    0, \text{benign}
    \end{cases} ,
\end{equation}

Unfortunately, developing such a classifier is notoriously hard under our considered threat model (\ie.,black-box, hard-label). Previous sample-wise black-box defenses~\citep{deepweep,frequency,rethinking,strip} only focus on the input space of $x$ through conducting various kinds of relevant transformation or augmentation techniques for $x$, thus fail to several advanced attacks~\citep{ISSBA,wanet} which embeds semantic features into the triggers.      
